Bringing the Galaxy's dark halo to life

We present a new method to construct fully self-consistent equilibrium models of multi-component disc galaxies similar to the Milky Way. We define distribution functions for the stellar disc and dark halo that depend on phase space position only through action coordinates. We then use an iterative approach to find the corresponding gravitational potential. We study the adiabatic response of the initially spherical dark halo to the introduction of the baryonic component and find that the halo flattens in its inner regions with final minor-major axis ratios $q$ = 0.75 - 0.95. The extent of the flattening depends on the velocity structure of the halo particles with radially biased models exhibiting a stronger response. In this latter case, which is according to cosmological simulations the most likely one, the new density structure resembles a "dark disc" superimposed on a spherical halo. We discuss the implications of these results for our recent estimate of the local dark matter density. The velocity distribution of the dark-matter particles near the Sun is very non-Gaussian. All three principal velocity dispersions are boosted as the halo contracts, and at low velocities a plateau develops in the distribution of $v_z$. For models similar to a state-of-the-art Galaxy model we find velocity dispersions around 155 km s$^{-1}$ for $v_z$ and the tangential velocity, $v_\varphi$, and 140 - 175 km s$^{-1}$ for the in-plane radial velocity, $v_R$, depending on the anisotropy of the model.

==> macros.tex <==
%%%%% AUTHORS - PLACE YOUR OWN MACROS HERE %%%%%
\arraycolsep0.35mm                      % makes multiple equations look nice
\catcode`\@=11
\def\gta{\ifmmode{\,\mathrel{\mathpalette\@versim>\,}}
    \else{$\,\mathrel{\mathpalette\@versim>}\,$}\fi}
\def\lta{\ifmmode{\,\mathrel{\mathpalette\@versim<\,}}
    \else{$\,\mathrel{\mathpalette\@versim<}\,$}\fi}
\def\@versim#1#2{\lower 2.9truept \vbox{\baselineskip 0pt \lineskip
    0.5truept \ialign{$\m@th#1\hfil##\hfil$\crcr#2\crcr\sim\crcr}}}
\catcode`\@=12  
%%%%%%%%%%%%%%%%%%%
% My own definitions
\renewcommand{\[}{\begin{equation}}
\renewcommand{\]}{\end{equation}}
% Bold face Greek letters
%
\font\gkvecten=cmmib10
\font\gkvecseven=cmmib7
\let\boldgrk=\gkvecten
\let\boldgrksc=\gkvecseven

\def\gkthing#1{{\mathchoice%
	{\hbox{{\boldgrk\char#1}}}
	{\hbox{{\boldgrk\char#1}}}
	{\hbox{{\boldgrksc\char#1}}}
	{\hbox{{\boldgrksc\char#1}}}}}
\def\rms{{\sc rms}}
\def\valpha{\gkthing{11}}
\def\vbeta{\gkthing{12}}
\def\vgamma{\gkthing{13}}
\def\vdelta{\gkthing{14}}
\def\vepsilon{\gkthing{15}}
\def\vzeta{\gkthing{16}}
\def\veta{\gkthing{17}}
\def\vtheta{\gkthing{18}}
\def\viotaeta{\gkthing{19}}
\def\vkappa{\gkthing{20}}
\def\vlambda{\gkthing{21}}
\def\vmu{\gkthing{22}}
\def\vnu{\gkthing{23}}
\def\vxi{\gkthing{24}}
\def\vpi{\gkthing{25}}
\def\vrho{\gkthing{26}}
\def\vsigma{\gkthing{27}}
\def\vtau{\gkthing{28}}
\def\vupsilon{\gkthing{29}}
\def\vphi{\gkthing{30}}
\def\vchi{\gkthing{31}}
\def\vpsi{\gkthing{32}}
\def\vomega{\gkthing{33}}
{\newif\ifnotend
\notendtrue
\def\veclist{ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrstuvwxyz.}
\def\top#1#2.{#1}
\def\tail#1#2.{#2.}
\loop\expandafter\xdef\csname v\expandafter\top\veclist\endcsname%
{{\noexpand\bf\expandafter\top\veclist}}
\edef\veclist{\expandafter\tail\veclist}
\if\veclist.\notendfalse\fi\ifnotend\repeat}
{\newif\ifnotend
\notendtrue
\def\veclist{ABCDEFGHIJKLMNOPQRSTUVWXYZ.}
\def\top#1#2.{#1}
\def\tail#1#2.{#2.}
\loop\expandafter\xdef\csname c\expandafter\top\veclist\endcsname%
{{\noexpand\cal\expandafter\top\veclist}}
\edef\veclist{\expandafter\tail\veclist}
\if\veclist.\notendfalse\fi\ifnotend\repeat}
\def\amoeba{{\sc amoeba}}
\def\i{{\rm i}}
\def\df{{\sc df}}\def\edf{{\sc edf}}
\def\DM{{\sc dm}}
\def\cE{{\cal E}}
\def\SN{S_{\rm N}}
\def\Teff{T_{\rm eff}}
\def\logg{\log g}
\def\feh{[{\rm Fe/H}]}\def\afe{[\alpha/{\rm Fe}]}
\def\vlos{v_{\rm los}}
\def\fracj#1#2{{\textstyle{#1\over#2}}}
\def\pa{\partial}
\def\ex#1{\left\langle#1\right\rangle}
\def\Rc{R_{\rm c}}\def\vc{v_{\rm c}}
\def\Rd{R_{\rm d}}
\def\Phic{\Phi_{\rm c}}
\def\Phieff{\Phi_{\rm eff}}
\def\mas{\,{\rm mas}}
\def\km{\,{\rm km}}
\def\cm{\,{\rm cm}}
\def\kms{\,{\rm km}\,{\rm s}^{-1}}
\def\mag{\,{\rm mag}}
\def\Myr{\,{\rm Myr}}
\def\yr{\,{\rm yr}}
\def\sec{\,{\rm s}}
\def\Gyr{\,{\rm Gyr}}
\def\K{\,{\rm K}} \let\kelvin=\K
\def\pc{\,{\rm pc}}
\def\kpc{\,{\rm kpc}}
\def\ergs{\,{\rm erg}}
\def\hi{H\,{\sc i}}
\def\e{{\rm e}}
\def\rd{{\rm d}}
\def\msun{\,{\rm M}_\odot}
\def\Lsun{\,{\rm L}_\odot}
\def\Fe{{\rm Fe}}
\def\meh{\hbox{[Me/H]}}
\def\feh{\hbox{[Fe/H]}}
\def\cafe{[\hbox{Ca}/\hbox{Fe}]}
\def\ofe{[\hbox{O}/\hbox{Fe}]}
\def\zeh{\hbox{[$Z$/H]}}
\def\alphaH{[\alpha/\hbox{H}]}
\def\afe{[\alpha/\hbox{Fe}]}
\def\HI{H\texttt{I}}
\def\dex{\,{\rm dex}}
\def\Rg{R_{\rm g}}
\def\vpbar{\overline{v}_\phi}
\def\figref#1{Fig.~\ref{#1}}
%%%%
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}

%%%%%%
\def\rhodm{\rho_{\rm dm,\odot}}
\def\zthin{z_{\rm thn}}
\def\zthick{z_{\rm thk}}
\def\fthick{f_{\rm thk}}
\def\d{\mathrm{d}}

\defcitealias{Juric2008}{J08}
\def\citetJuric{\citetalias{Juric2008}}
\def\citepJuric{\citepalias{Juric2008}}


\newcommand*\aap{A\&A}
\let\astap=\aap
\newcommand*\aapr{A\&A~Rev.}
\newcommand*\aaps{A\&AS}
\newcommand*\actaa{Acta Astron.}
\newcommand*\aj{AJ}
\newcommand*\ao{Appl.~Opt.}
\let\applopt\ao
\newcommand*\apj{ApJ}
\newcommand*\apjl{ApJ}
\let\apjlett\apjl
\newcommand*\apjs{ApJS}
\let\apjsupp\apjs
\newcommand*\aplett{Astrophys.~Lett.}
\newcommand*\apspr{Astrophys.~Space~Phys.~Res.}
\newcommand*\apss{Ap\&SS}
\newcommand*\araa{ARA\&A}
\newcommand*\azh{AZh}
\newcommand*\baas{BAAS}
\newcommand*\bac{Bull. astr. Inst. Czechosl.}
\newcommand*\bain{Bull.~Astron.~Inst.~Netherlands}
\newcommand*\caa{Chinese Astron. Astrophys.}
\newcommand*\cjaa{Chinese J. Astron. Astrophys.}
\newcommand*\fcp{Fund.~Cosmic~Phys.}
\newcommand*\gca{Geochim.~Cosmochim.~Acta}
\newcommand*\grl{Geophys.~Res.~Lett.}
\newcommand*\iaucirc{IAU~Circ.}
\newcommand*\icarus{Icarus}
\newcommand*\jcap{J. Cosmology Astropart. Phys.}
\newcommand*\jcp{J.~Chem.~Phys.}
\newcommand*\jgr{J.~Geophys.~Res.}
\newcommand*\jqsrt{J.~Quant.~Spec.~Radiat.~Transf.}
\newcommand*\jrasc{JRASC}
\newcommand*\memras{MmRAS}
\newcommand*\memsai{Mem.~Soc.~Astron.~Italiana}
\newcommand*\mnras{MNRAS}
\newcommand*\na{New A}
\newcommand*\nar{New A Rev.}
\newcommand*\nat{Nature}
\newcommand*\nphysa{Nucl.~Phys.~A}
\newcommand*\pasa{PASA}
\newcommand*\pasj{PASJ}
\newcommand*\pasp{PASP}
\newcommand*\physrep{Phys.~Rep.}
\newcommand*\physscr{Phys.~Scr}
\newcommand*\planss{Planet.~Space~Sci.}
\newcommand*\pra{Phys.~Rev.~A}
\newcommand*\prb{Phys.~Rev.~B}
\newcommand*\prc{Phys.~Rev.~C}
\newcommand*\prd{Phys.~Rev.~D}
\newcommand*\pre{Phys.~Rev.~E}
\newcommand*\prl{Phys.~Rev.~Lett.}
\newcommand*\procspie{Proc.~SPIE}
\newcommand*\qjras{QJRAS}
\newcommand*\rmxaa{Rev. Mexicana Astron. Astrofis.}
\newcommand*\skytel{S\&T}
\newcommand*\solphys{Sol.~Phys.}
\newcommand*\sovast{Soviet~Ast.}
\newcommand*\ssr{Space~Sci.~Rev.}
\newcommand*\zap{ZAp}
